Enhancing Image-Text Matching with Adaptive Feature Aggregation

Image-text matching aims to find matched cross-modal pairs accurately. While current methods often rely on projecting cross-modal features into a common embedding space, they frequently suffer from imbalanced feature representations across different modalities, leading to unreliable retrieval results. To address these limitations, we introduce a novel Feature Enhancement Module that adaptively aggregates single-modal features for more balanced and robust image-text retrieval. Additionally, we propose a new loss function that overcomes the shortcomings of original triplet ranking loss, thereby significantly improving retrieval performance. The proposed model has been evaluated on two public datasets and achieves competitive retrieval performance when compared with several state-of-the-art models. Implementation codes can be found here.

==> icassp_2024_7903_arxiv_submission/tables/table_ablation_study.tex <==
\begin{table}[htbp]
  \centering
  \fontsize{8}{3}\selectfont
  \caption{Ablation studies on Flickr30K. {(I)}: Feature extractor and triplet ranking loss~\cite{faghri2018vse++}. {(II)}: Feature aggregation module; {(III)}: Feature selection module; {(IV)}: The new loss function.}
  {
    \tabcolsep 2pt
    \begin{tabu}{@{\;} cccc @{\quad} ccccccc @{\;}}
        \toprule
        \multicolumn{4}{l}{\bf Datasets} & \multicolumn{7}{c}{\bf Flickr30K 1K Test} \\ 
        %\cmidrule(lr){6-12}
        \multicolumn{4}{l}{Tasks} & \multicolumn{3}{c}{image-to-text} & \multicolumn{3}{c}{text-to-image} \\
        %\cmidrule(lr){6-8} \cmidrule(lr){9-11}
        % \\[-0.6ex]
        (I) & (II) & (III) & (IV) & \textsc{R@1} & \textsc{R@5} & \textsc{R@10} & \textsc{R@1} & \textsc{R@5} & \textsc{R@10} & {\textsc{rSum}} \\
        \hline \\[-0.5ex]
        \rowcolor{Gray}          
        \checkmark & \checkmark & \checkmark & \checkmark & 81.8 & 95.8 & 98.1 & 59.9 & 84.9 & 91.2 & 510.9 \\
        \hline \\[-0.5ex]
        \checkmark & \checkmark & \checkmark & & 79.4 & 94.7 & 97.1 & 59.1 & 84.0 & 89.6 & 503.8  \\
        \checkmark & \checkmark & & & 75.3 & 92.1 & 95.7 & 57.1 & 82.7 & 89.4 & 492.4  \\
        \checkmark & & & & 70.3 & 91.0 & 95.5 & 51.9 & 79.0 & 87.2 & 474.9 \\   
        \bottomrule
  \end{tabu}
}
\label{tab:t3}
\end{table}












% original one

% \begin{table*}[t]
%     \centering
%     \small
%   \caption{Ablation studies on Flickr30K and MS-COCO; BASE: Feature extractor (BUTD, BERT) + Triplet ranking loss~\cite{faghri2018vse++}. Projector: feature projector; Enhancement: feature enhancement; NewLoss: the proposed new loss function.}.
%     \resizebox{\textwidth}{!}
%     {
%       \tabcolsep 1.5pt
%       \begin{tabu}{@{\;} lcccc @{\quad} ccccccc ccccccc @{\;}}
%           \toprule
  
%           {Datasets} & & & & & \multicolumn{7}{c}{Flickr30$\mathrm{K}$ 1$\mathrm{K}$ Test} &
%           \multicolumn{7}{c}{MS-COCO 5-fold 1$\mathrm{K}$ Test} \\ 
%           \cmidrule(lr){6-12} \cmidrule(lr){13-19}
%           {Tasks} & & & & & \multicolumn{3}{c}{image-to-text} & \multicolumn{3}{c}{text-to-image} & & \multicolumn{3}{c}{image-to-text} & \multicolumn{3}{c}{text-to-image} \\
%           \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){13-15} \cmidrule(lr){16-18}
%           Index & {BASE} & Project & Enhancement & NewLoss & \textsc{R@1} & \textsc{R@5} & \textsc{R@10} & \textsc{R@1} & \textsc{R@5} & \textsc{R@10} & {\textsc{rSum}$\uparrow$} & \textsc{R@1} & \textsc{R@5} & \textsc{R@10} & \textsc{R@1} & \textsc{R@5} & \textsc{R@10} & \textsc{rSum}$\uparrow$ \\
%           \midrule
%           \rowcolor{Gray}          
%           0 & \checkmark & \checkmark & \checkmark & \checkmark & {98.8} & {99.6} & {99.9} & {92.4} & {98.3} & {99.0} & 588.0 & {96.5} & {99.3} & {99.8} & {89.5} & {96.5} & {97.8} & 579.4 \\
%           \midrule
%           1 & \checkmark & \checkmark & \checkmark & & 97.5 & 99.6 & 99.8 & 86.0 & 94.9 & 96.7 & 574.5 & 96.1 & 99.1 & 99.7 & 86.6 & 94.6 & 96.4 & 572.6 \\
%           2 & \checkmark & \checkmark & & & 97.4 & 99.6 & 99.9 & 79.2 & 86.9 & 89.3 & 552.3 & 83.3 & 96.4 & 98.6 & 63.4& 90.0 & 95.3 & 527.0 \\
%           3 & \checkmark & & & & 53.4 & 80.2 & 87.8 & 37.8 & 68.6 & 80.1 & 407.9 & 28.4 & 55.3 & 71.8 & 33.7 & 69.1 & 82.2 & 340.5 \\   
%           \bottomrule
%     \end{tabu}
%   }
%   \label{tab:t3}
%   \end{table*}



==> icassp_2024_7903_arxiv_submission/tables/table_coco_5k.tex <==
\begin{table}[t]
    \centering
    \fontsize{8}{3}\selectfont
    \caption{Results on MS-COCO 5K. The best and second best results (in \textsc{rSum}) except ours are highlighted in \textbf{bold} and \underline{underline}. --: Results are missing from their publications. }
    %\resizebox{\textwidth}{!}
    \tabcolsep 3.5pt
    \begin{tabular}{@{\;}l@{\quad}ccccccc@{\;}}
         \toprule
         {\bf Datasets} & \multicolumn{7}{c}{\bf MS-COCO 5K Test}\\
         %\cmidrule(lr){2-8}
         {Tasks}  & \multicolumn{3}{c}{image-to-text} & \multicolumn{3}{c}{text-to-image} \\
         %\cmidrule(lr){2-4} \cmidrule(lr){5-7}
         {Method} & \textsc{R@1} & \textsc{R@5} & \textsc{R@10} & \textsc{R@1} & \textsc{R@5} & \textsc{R@10} & \textsc{rSum} \\
         \hline \\[-0.5ex] 
        VSE++ & 41.3 & 71.1 & 81.2 & 30.3 & 59.4 & 72.4 & 355.7 \\
         %SCO{\tiny 2018} & 42.8 & 72.3 & 83.0 & 33.1 & 62.9 & 75.5 & 369.6 \\
         SCAN & 50.4 & 82.2 & 90.0 & 38.6 & 69.3 & 80.4 & 410.9 \\
         VSRN & 53.0 & 81.1 & 89.4 & 40.5 & 70.6 & 81.1 & 415.7 \\
         %{CAMERA*}{\tiny 2020} & 55.1 & 82.9 & 91.2 & 40.5 & 71.7 & 82.5 & 423.9 \\
         %VSE$\infty$*{\tiny 2021} & 68.1 & 90.2 & 95.2 & 52.7 & 80.2 & 88.3 & \color{red}{474.8} \\
         SGRAF & 57.8 & -- & \underline{91.6} & \textbf{41.9} & -- & 81.3 & -- \\
         RCAR & 57.4 & 83.8 & 91.0 & 40.7 & 69.8 & 80.4 & 423.1 \\
         %CMCAN{\tiny 2022} & 61.5 & -- & 92.9 & 44.0 & -- & 82.6 & -- \\
         %MV-VSE{\tiny 2022} & 59.1 & 86.3 & 92.5 & 42.5 & 72.8 & 83.1 & \color{blue}{436.3} \\
         DivEmbed & \underline{58.8} & \underline{84.9} & 91.5 & 41.1 & 72.0 & \textbf{82.4} & \underline{430.7} \\
         {{\textbf {Ours}}} & \textbf{59.3} & \textbf{85.9} & \textbf{92.3} & \underline{41.4} & \textbf{72.0} & \underline{82.3} & \textbf{433.2} \\   
         %{\scriptsize {\textbf {MinMa-2 (Ours)}}} & \textbf{90.5} & \textbf{96.4} & \textbf{97.6} & \textbf{81.0} & \textbf{91.5} & \textbf{93.9} & \textbf{551.0} \\   
         \bottomrule
    \end{tabular}
    \label{tab:t2}
\end{table}

==> icassp_2024_7903_arxiv_submission/tables/table_f30k_coco.tex <==
\begin{table*}[htbp]
    \centering
    \fontsize{3}{3}\selectfont
    % \tiny
    \caption{Retrieval results of state-of-the-art methods on Flickr30K and MS-COCO. The best and second best results (in \textsc{rSum}) are highlighted in \textbf{bold} and \underline{underline}.}
    \resizebox{\textwidth}{!}
    {
      \tabcolsep 2pt
      \begin{tabu} {@{\;} l @{\quad} ccccccc ccccccc@{\;}}
          \hline \\[-1.5ex]
  
          {\bf Datasets} & \multicolumn{7}{c}{\bf Flickr30K 1K Test} &
          \multicolumn{7}{c}{\bf MS-COCO 5-fold 1K Test} \\ 
          %\cmidrule(lr){2-8} \cmidrule(lr){9-15}
          %\hline
          {Tasks} & \multicolumn{3}{c}{image-to-text} & \multicolumn{3}{c}{text-to-image} & & \multicolumn{3}{c}{image-to-text} & \multicolumn{3}{c}{text-to-image} \\
          % \midrule
          %\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
          {Methods} & \textsc{R@1} & \textsc{R@5} & \textsc{R@10} & \textsc{R@1} & \textsc{R@5} & \textsc{R@10} & {\textsc{rSum}} & \textsc{R@1} & \textsc{R@5} & \textsc{R@10} & \textsc{R@1} & \textsc{R@5} & \textsc{R@10} & \textsc{rSum} \\
          \hline \\[-1.5ex] 
           {VSE++~\cite{faghri2018vse++} \textsubscript{2018}} & {52.9} & {80.5} & {87.2} & {39.6} & {70.1} & {79.5} & {409.8} & {64.6} & {90.0} & {95.7} & {52.0} & {84.3} & {92.0} & {478.6} \\
          %{SCO~\cite{Huang2018}\textsubscript{2018}} & {55.5} & {82.0} & {89.3} & {41.4} & {70.5} & {80.1} & {418.5} & {69.9} & {92.9} & {97.5} & {56.7} & {87.5} & {94.8} & {499.3} \\
          %  \hline
           {SCAN~\cite{LeeCHHH18} \textsubscript{2018}} & {67.4} & {90.3} & {95.8} & {48.6} & {77.7} & {85.2} & {465.0} & {72.7} & {94.8} & {98.4} & {58.8} & {88.4} & {94.8} & {507.9} \\
           %{LIWE~\cite{WehrmannLSB19} \textsubscript{2019}} & {69.6} & {90.3} & {95.6} & {51.2} &  {80.4} & {87.2} & {474.3} & {73.2} & {95.5} & {98.2} & {57.9} & {88.3} & {94.5} & {507.6} \\
           {VSRN~\cite{LiZLLF19}\textsubscript{2019}} & {71.3} & {90.6} & {96.0} & {54.7} & {81.8} & {88.2} & {482.6} & {76.2} & {94.8} & {98.2} & {62.8} & {89.7} & {95.1} & {516.8} \\
           {CVSE~\cite{WangZJPM20} \textsubscript{2020}} & {70.5} & {88.0} & {92.7} & {54.7} & {82.2} & {88.6} & {476.7} & {69.2} & {93.3} & {97.5} & {55.7} & {86.9} & {93.8} & {496.4} \\
           {SGRAF~\cite{DiaoZML21} \textsubscript{2021}} & {77.8} & {94.1} & {97.4} & \underline{58.5} & {83.0} & {88.8} & {499.6} & {79.6} & {96.2} & {98.5} & {63.2} & {90.7} & \textbf{96.1} & {524.3} \\ 
           %SHAN*\cite{JiCW21}\textsubscript{2021} & 74.6 & 93.5 & 96.9 & 55.3 & 81.3 & 88.4 & 490.0 & 76.8 & 96.3 & 98.7 & 62.6 & 89.6 & 95.8 & 519.8 \\
           %MV-VSE~\cite{LiGFHX22}\textsubscript{2022} & {79.0} & {94.9} & {97.7} & {59.1} & {84.6} & {90.6} & {505.8} & {78.7} & {95.7} & {98.7} & {62.7} & {90.4} & {95.7} & {521.9} \\ 
           %CMCAN~\cite{ZhangMZ022} \textsubscript{2022} & {79.5} & {95.6} & {97.6} & \textbf{60.9} & {84.3} & {89.9} & {507.8} & {81.2} & {96.8} & {98.7} & {65.4} & {91.0} & {96.2} & \color{blue}{529.3} \\ 
           %GraDual*~\cite{LongHWP22}\textsubscript{2022} & 78.3 & 96.0 & 98.0 & 60.4 & 86.7 & 92.0 & 511.4 & 77.0 & 96.4 & 98.6 & 65.3 & 91.9 & 96.4 & 525.6 \\ 
          %\midrule
          % \hline
          % CAMERA*~\cite{Qu0CN020}\textsubscript{2020} & {78.0} & {95.1} & {97.9} & {60.3} & {85.9} & {91.7} & {508.9} & {77.5} & {96.3} & {98.8} & {63.4} & {90.9} & {95.8} & {522.7} \\ 
          %VSE$\infty$\cite{ChenH0JW21}\textsubscript{2021} & {81.7} & {95.4} & {97.6} & {61.4} & {85.9} & {91.5} & {513.5} & {79.7} & {96.4} & {98.9} & {64.8} & {91.4} & {96.3} & {527.5} \\ 
          % MV-VSE~\cite{LiGFHX22}\textsubscript{2022} & {82.1} & {95.8} & {97.9} & {63.1} & {86.7} & {92.3} & \color{blue}{517.5} & {80.4} & {96.6} & {99.0} & {64.9} & {91.2} & {96.0} & {528.1} \\
          % VSE$\infty$*\cite{ChenH0JW21}\textsubscript{2021} & {88.7} & {98.9} & {99.8} & {76.1} & {94.5} & {97.1} & {\color{red}{555.1}} & {85.6} & {98.0} & {99.4} & {73.1} & {94.3} & {97.7} & \color{red}{548.1} \\
          GraDual~\cite{LongHWP22} \textsubscript{2022} & 76.1 & \underline{94.7} & \underline{97.7} & 57.7 & \underline{84.1} & \underline{90.5} & 500.8 & 76.8 & 95.9 & 98.3 & \underline{63.7} & 90.8 & 95.6 & 521.1 \\
          RCAR~\cite{DiaoZLRL23} \textsubscript{2023} & 77.8 & 93.6 & 96.9 & 57.2 & 82.8 & 88.5 & 496.8 & 78.2 & \underline{96.3} & 98.4 & 62.2 & 89.6 & 95.3 & 520.0 \\
          DivEmbed~\cite{KimKK23} \textsubscript{2023} & \underline{77.8} & 94.0 & 97.5 & 57.5 & 84.0 & 90.0 & \underline{500.8} & \underline{79.9} & 96.2 & \underline{98.6} & 63.6 & \underline{90.7} & 95.7 & \underline{524.6} \\ 
          %\hline \\[-1.5ex]
          \rowcolor{Gray}
          \textbf{Ours} & \textbf{81.8} & \textbf{95.8} & \textbf{98.1} & \textbf{59.9} & \textbf{84.9} & \textbf{91.2} & {\textbf{510.9}} & \textbf{80.1} & \textbf{96.3} & \textbf{98.7} & \textbf{64.0} & \textbf{90.9} & \underline{96.0} & \textbf{526.1} \\
          % \textbf{MiMa-2 (Ours)} & \textbf{98.8} & \textbf{99.6} & \textbf{99.9} & \textbf{92.4} & \textbf{98.3} & \textbf{99.0} & {\textbf{588.0}} & \textbf{96.5} & \textbf{99.3} & \textbf{99.8} & \textbf{89.5} & \textbf{96.5} & \textbf{97.8} & \textbf{579.4} \\
          \hline
    \end{tabu}
  }
  \label{tab:t1}
  \end{table*}
